Utilize the Flow before Stepping into the Same River Twice: Certainty Represented Knowledge Flow for Refusal-Aware Instruction Tuning

Refusal-Aware Instruction Tuning (RAIT) enables Large Language Models (LLMs) to refuse to answer unknown questions. By modifying responses of unknown questions in the training data to refusal responses such as "I don't know", RAIT enhances the reliability of LLMs and reduces their hallucination. Generally, RAIT modifies training samples based on the correctness of the initial LLM's response. However, this crude approach can cause LLMs to excessively refuse answering questions they could have correctly answered, the problem we call over-refusal. In this paper, we explore two primary causes of over-refusal: Static conflict occurs when similar samples within the LLM's feature space receive differing supervision signals (original vs. modified "I don't know"). Dynamic conflict arises as the LLM's evolving knowledge during SFT enables it to answer previously unanswerable questions, but the now-answerable training samples still retain the original "I don't know" supervision signals from the initial LLM state, leading to inconsistencies. These conflicts cause the trained LLM to misclassify known questions as unknown, resulting in over-refusal. To address this issue, we introduce Certainty Represented Knowledge Flow for Refusal-Aware Instructions Tuning (CRaFT). CRaFT centers on two main contributions: First, we additionally incorporate response certainty to selectively filter and modify data, reducing static conflicts. Second, we implement preliminary rehearsal training to characterize changes in the LLM's knowledge state, which helps mitigate dynamic conflicts during the fine-tuning process. We conducted extensive experiments on open-ended question answering and multiple-choice question task. Experiment results show that CRaFT can improve LLM's overall performance during the RAIT process. Code and data will be released at https://github.com/opendatalab/CRaFT .

==> table/ab_MCQA_llama2.tex <==
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}

\begin{table}[t]
\centering
{\fontsize{9pt}{11pt}\selectfont
\label{table:ab_exp_MCQA}
\begin{tabular}{|c|ll|ll|}
\hline
\multicolumn{1}{|l|}{}  & \multicolumn{2}{c|}{\textbf{MMLU (ID)}}                                 & \multicolumn{2}{c|}{\textbf{ARC-c (OOD)}}                               \\ \hline
\textbf{Method}         & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\textbf{Cor-RAIT}       & \multicolumn{1}{l|}{39.57}          & 11.32                             & \multicolumn{1}{l|}{38.14}          & 11.08                             \\ \hline
\textbf{CRaFT w/o Flow} & \multicolumn{1}{l|}{31.01}         & 12.97                             & \multicolumn{1}{l|}{32.34}          & 13.45                             \\ \hline
\textbf{CRaFT w/o Cer}  & \multicolumn{1}{l|}{32.05}          & 11.51                             & \multicolumn{1}{l|}{32.94}          & 13.85                             \\ \hline
\textbf{CRaFT}          & \multicolumn{1}{l|}{36.39}          & 12.46                             & \multicolumn{1}{l|}{35.92}          & 12.58                             \\ \hline
\end{tabular}
}
\caption{Ablation Experiment Results in MCQA Task}
\vspace{-10pt}
\end{table}
\endgroup  % End the group

==> table/ab_OEQA_llama2.tex <==
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}

\begin{table}[t]
\centering
\label{table:ab_exp_OEQA}
{\fontsize{9pt}{11pt}\selectfont
\begin{tabular}{|c|ll|ll|}
\hline
\multicolumn{1}{|l|}{}  & \multicolumn{2}{c|}{\textbf{TriviaQA (ID)}}                             & \multicolumn{2}{c|}{\textbf{NQ (OOD)}}                                  \\ \hline
\textbf{Method}         & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS$\uparrow$}} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS$\uparrow$}} \\ \hline
\textbf{Cor-RAIT}       & \multicolumn{1}{l|}{18.32}          & 19.73                             & \multicolumn{1}{l|}{27.59}          & 4.71                              \\ \hline
\textbf{CRaFT w/o Flow} & \multicolumn{1}{l|}{20.45}          & 21.12                             & \multicolumn{1}{l|}{38.75}          & 5.15                              \\ \hline
\textbf{CRaFT w/o Cer}  & \multicolumn{1}{l|}{15.65}          & 20.11                             & \multicolumn{1}{l|}{22.13}          & 5.42                              \\ \hline
\textbf{CRaFT}          & \multicolumn{1}{l|}{12.93}         & 23.29                             & \multicolumn{1}{l|}{22.38}          & 6.54                              \\ \hline
\end{tabular}
}
\caption{Ablation Experiment Results in OEQA Task.}
\end{table}
\endgroup  % End the group

==> table/main_MCQA_ALL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[t]
\label{table:main_exp_MCQA}
\centering
{\fontsize{9pt}{11pt}\selectfont
\begin{tabular}{|c|c|lll|lll|}
\hline
\multicolumn{1}{|l|}{}                                                                  & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{3}{c|}{\textbf{MMLU (ID)}}                                                                       & \multicolumn{3}{c|}{\textbf{ARC-c (OOD)}}                                                                     \\ \hline
\textbf{Model}                                                                          & \textbf{Method}                & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama2-\\ 7B-\\Chat\end{tabular}}}     & \textbf{Init-Basic}            & \multicolumn{1}{l|}{\textbf{45.6}}  & \multicolumn{1}{l|}{52.8}           & 0                                 & \multicolumn{1}{l|}{53.9}           & \multicolumn{1}{l|}{46}             & 0                        \\ \cline{2-8} 
                                                                                        & \textbf{Init-Refuse}           & \multicolumn{1}{l|}{36.4}           & \multicolumn{1}{l|}{38.9}           & 3.9                               & \multicolumn{1}{l|}{44.4}           & \multicolumn{1}{l|}{\textbf{35.7}}  & 2.6                               \\ \cline{2-8} 
                                                                                        & \textbf{Van-Tuning}            & \multicolumn{1}{l|}{47}             & \multicolumn{1}{l|}{53.1}           & 1.2                               & \multicolumn{1}{l|}{54.5}           & \multicolumn{1}{l|}{45.5}           & 1.2                               \\ \cline{2-8} 
                                                                                        & \textbf{Cor-RAIT}              & \multicolumn{1}{l|}{44.5}           & \multicolumn{1}{l|}{39.6}           & 11.3                              & \multicolumn{1}{l|}{\textbf{55.8}}  & \multicolumn{1}{l|}{38.1}           & 11.1                              \\ \cline{2-8} 
                                                                                        & \textbf{CRaFT}                 & \multicolumn{1}{l|}{43.9}           & \multicolumn{1}{l|}{\textbf{36.4}}  & \textbf{12.5}                     & \multicolumn{1}{l|}{54.7}           & \multicolumn{1}{l|}{35.9}           & \textbf{12.6}                     \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3-\\ 8B-\\Instruct\end{tabular}}} & \textbf{Init-Basic}            & \multicolumn{1}{l|}{66.8}           & \multicolumn{1}{l|}{33.1}           & 0                                 & \multicolumn{1}{l|}{\textbf{80.6}}  & \multicolumn{1}{l|}{19.5}           & 0                                 \\ \cline{2-8} 
                                                                                        & \textbf{Init-Refuse}           & \multicolumn{1}{l|}{50}             & \multicolumn{1}{l|}{17}             & 15.7                              & \multicolumn{1}{l|}{65.3}           & \multicolumn{1}{l|}{14.4}           & 5.6                               \\ \cline{2-8} 
                                                                                        & \textbf{Van-Tuning}            & \multicolumn{1}{l|}{\textbf{69.5}}  & \multicolumn{1}{l|}{30.5}           & 8                                 & \multicolumn{1}{l|}{80.3}           & \multicolumn{1}{l|}{19.7}           & -1.3                              \\ \cline{2-8} 
                                                                                        & \textbf{Cor-RAIT}              & \multicolumn{1}{l|}{63.9}           & \multicolumn{1}{l|}{21.6}           & 20.4                              & \multicolumn{1}{l|}{79.4}           & \multicolumn{1}{l|}{16.2}           & 12.2                              \\ \cline{2-8} 
                                                                                        & \textbf{CRaFT}                 & \multicolumn{1}{l|}{53.3}           & \multicolumn{1}{l|}{\textbf{9.6}}   & \textbf{34}                       & \multicolumn{1}{l|}{74.1}           & \multicolumn{1}{l|}{\textbf{12.7}}  & \textbf{21.4}                     \\ \hline
\end{tabular}
}
\caption{Experimental Results in MCQA Task.}
\vspace{-10pt}
\end{table}
\endgroup  % End the group

==> table/main_OEQA_ALL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begingroup
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{1mm}
\begin{table}[t]
\label{table:main_exp_OEQA}
\centering
{\fontsize{9pt}{11pt}\selectfont
\begin{tabular}{|cc|lll|lll|}
\hline
\multicolumn{2}{|l|}{}                                                                                                               & \multicolumn{3}{c|}{\textbf{TriviaQA (ID)}}                                                                   & \multicolumn{3}{c|}{\textbf{NQ (OOD)}}                                                                        \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}}                                                                          & \textbf{Method}      & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_c$}$\uparrow$} & \multicolumn{1}{c|}{\textbf{$P_w$}$\downarrow$} & \multicolumn{1}{c|}{\textbf{THS}$\uparrow$} \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama2-\\ 7B-\\Chat\end{tabular}}}}     & \textbf{Init-Basic}  & \multicolumn{1}{l|}{\textbf{54}}             & \multicolumn{1}{l|}{46}             & 0                                 & \multicolumn{1}{l|}{\textbf{29.3}}           & \multicolumn{1}{l|}{70.7}           & 0                                 \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Init-Refuse} & \multicolumn{1}{l|}{37}             & \multicolumn{1}{l|}{21.7}           & 11.5                              & \multicolumn{1}{l|}{20.8}           & \multicolumn{1}{l|}{38.6}           & 4.8                               \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Van-Tuning}  & \multicolumn{1}{l|}{48.6}           & \multicolumn{1}{l|}{44.5}           & -3.7                              & \multicolumn{1}{l|}{18.3}           & \multicolumn{1}{l|}{50.2}           & -2.5                              \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Cor-RAIT}    & \multicolumn{1}{l|}{41.3}           & \multicolumn{1}{l|}{18.3}           & 19.7                              & \multicolumn{1}{l|}{16.2}           & \multicolumn{1}{l|}{27.6}           & 4.7                               \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{CRaFT}       & \multicolumn{1}{l|}{38.5}           & \multicolumn{1}{l|}{\textbf{12.9}}           & \textbf{23.3}                              & \multicolumn{1}{l|}{15.8}           & \multicolumn{1}{l|}{\textbf{22.4}}           & \textbf{6.5}                               \\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3-\\ 8B-\\Instruct\end{tabular}}}} & \textbf{Init-Basic}  & \multicolumn{1}{l|}{\textbf{66.8}}           & \multicolumn{1}{l|}{33.2}           & 0                                 & \multicolumn{1}{l|}{\textbf{40.3}}           & \multicolumn{1}{l|}{59.7}           & 0                                 \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Init-Refuse} & \multicolumn{1}{l|}{53.9}           & \multicolumn{1}{l|}{20.8}           & 12                                & \multicolumn{1}{l|}{31.1}           & \multicolumn{1}{l|}{38.6}           & \textbf{5}                                 \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Van-Tuning}  & \multicolumn{1}{l|}{55}             & \multicolumn{1}{l|}{38.1}           & -21.9                             & \multicolumn{1}{l|}{21}             & \multicolumn{1}{l|}{48.5}           & -11.7                             \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{Cor-RAIT}    & \multicolumn{1}{l|}{45.4}           & \multicolumn{1}{l|}{13.2}           & 18.8                              & \multicolumn{1}{l|}{17.2}           & \multicolumn{1}{l|}{\textbf{25.6}}           & -0.1                              \\ \cline{2-8} 
\multicolumn{1}{|c|}{}                                                                                        & \textbf{CRaFT}       & \multicolumn{1}{l|}{43.5}           & \multicolumn{1}{l|}{\textbf{10.9}}           & \textbf{21.5}                              & \multicolumn{1}{l|}{19}             & \multicolumn{1}{l|}{27.5}           & 0.4                               \\ \hline
\end{tabular}
}
\caption{Experimental Results in OEQA Task.}
\end{table}
\endgroup  % End the group
